Toward Efficient Automated Feature Engineering

Automated Feature Engineering (AFE) refers to automatically generate and select optimal feature sets for downstream tasks, which has achieved great success in real-world applications. Current AFE methods mainly focus on improving the effectiveness of the produced features, but ignoring the low-efficiency issue for large-scale deployment. Therefore, in this work, we propose a generic framework to improve the efficiency of AFE. Specifically, we construct the AFE pipeline based on reinforcement learning setting, where each feature is assigned an agent to perform feature transformation \com{and} selection, and the evaluation score of the produced features in downstream tasks serve as the reward to update the policy. We improve the efficiency of AFE in two perspectives. On the one hand, we develop a Feature Pre-Evaluation (FPE) Model to reduce the sample size and feature size that are two main factors on undermining the efficiency of feature evaluation. On the other hand, we devise a two-stage policy training strategy by running FPE on the pre-evaluation task as the initialization of the policy to avoid training policy from scratch. We conduct comprehensive experiments on 36 datasets in terms of both classification and regression tasks. The results show $2.9\%$ higher performance in average and 2x higher computational efficiency comparing to state-of-the-art AFE methods.

==> comparation.table.tex <==
\begin{table*}
\centering
\begin{tabular}{c|c|l|l|l|l|l|l|l|c}
\hline
Dataset & Source & C$\backslash$R & Instances$\backslash$Features & $\mathrm{AutoFS_{RD}}$ & $\mathrm{RTDL_{RN}}$  &  NFS  & $\TheName _{RL}$  & $\TheName _{RD}$  & \TheName \\
\hline
Higgs Boson & UCIrvine & C &   50000$\backslash$28  & 0.723 &  0.756 &  0.731 &  0.725 & 0.802 & \textbf{0.836} \\
\hline
% Amazon Employee & Kaggle & C  & 32769$\backslash$9  & 0.948 &  0.484 & 0.945 &  0.943 & 0.950 & \textbf{0.951} \\   
Amazon Employee & Kaggle & C  & 32769$\backslash$9  & 0.948 &  0.484 & 0.950 &  0.943 & 0.950 & \textbf{0.951} \\   
\hline
PimaIndian & UCIrvine & C & 768$\backslash$8 & 0.779 &  0.743   & 0.790 & 0.783 &  0.792 & \textbf{0.798}  \\ 
\hline
SpectF & UCIrvine & C & 267$\backslash$44  & 0.871 & 0.639  & 0.876  & 0.862 & 0.900 & \textbf{0.903} \\ 
\hline
% SVMGuide3 & LibSVM & C  & 1243$\backslash$21  & 0.852 & 0.728  & 0.865 & 0.861 &  0.875  & \textbf{0.881} \\ % 
SVMGuide3 & LibSVM & C  & 1243$\backslash$21  & 0.842 & 0.728  & 0.846 & 0.843 &  0.875  & \textbf{0.881} \\
\hline
% German Credit & UCIrvine & C & 1001$\backslash$24  & 0.775 & 0.681 & 0.805  & 0.800 &  0.810 & \textbf{0.816} \\  % 
German Credit & UCIrvine & C & 1001$\backslash$24  & 0.775 & 0.681 & 0.780  & 0.773 &  0.810 & \textbf{0.816} \\  % 
\hline
Bikeshare DC & Kaggle  & R & 10886$\backslash$11  & 0.978 & 0.945 & 0.990 & 0.983  &  0.992 & \textbf{0.993} \\  %  
\hline
% Housing Boston & UCIrvine & R  & 506$\backslash$13  & 0.709 & 0.648 & 0.686 & 0.683  &  0.798 & \textbf{0.836}    \\ %  
Housing Boston & UCIrvine & R  & 506$\backslash$13  & 0.709 & 0.648 & 0.710 & 0.693  &  0.798 & \textbf{0.821}    \\ %  
\hline
Airfoil & UCIrvine & R &  1503$\backslash$5  & 0.784 & 0.697 & 0.796  & 0.781 & 0.790  & \textbf{0.810} \\  %  
\hline
AP-omentum-ovary & OpenML & C  & 275$\backslash$10936  & 0.852 & 0.659 & 0.864  & 0.858 &  0.879 & \textbf{0.884} \\  % 
\hline
% Lymphography & UCIrvine & C  & 148$\backslash$18 & 0.895 & 0.000 & 0.929 & 0.921  &  0.960 & \textbf{0.964} \\  % 
Lymphography & UCIrvine & C  & 148$\backslash$18 & 0.895 & 0.000 & 0.922 & 0.921  &  0.960 & \textbf{0.964} \\  % 
\hline
% Ionosphere & UCIrvine & C  & 351$\backslash$34  & 0.958 & 0.883 & 0.969 & 0.964  &  0.973 & \textbf{0.977} \\  %    
Ionosphere & UCIrvine & C  & 351$\backslash$34  & 0.934 & 0.883 & 0.957 & 0.944  &  0.973 & \textbf{0.977} \\  %  
\hline
Openml 618 & OpenML &  R & 1000$\backslash$50  & 0.619 & 0.072 & 0.640  & 0.635  &  0.728 & \textbf{0.737}  \\ % 
\hline
Openml 589 & OpenML & R  & 1000$\backslash$25  & 0.737 & 0.578 & 0.754 & 0.748  &  0.757 & \textbf{0.764} \\  %   
\hline
Openml 616 & OpenML & R & 500$\backslash$50  & 0.609 &   0.000  & 0.673 & 0.653  & 0.675 & \textbf{0.689}  \\ %   this 0.000 is -0.0088
\hline
Openml 607 & OpenML & R  & 1000$\backslash$50  & 0.634 & 0.025 & 0.688 & 0.678  &  0.728 & \textbf{0.734} \\  % 
\hline
Openml 620 & OpenML & R  & 1000$\backslash$25  & 0.705 & 0.047 & 0.732 & 0.727  & 0.736  & \textbf{0.748} \\  % 
\hline
Openml 637 & OpenML &  R & 500$\backslash$50  & 0.608 & 0.016  & 0.634 &  0.633  &  0.624 & \textbf{0.646}  \\ % 
\hline
Openml 586 & OpenML & R  & 1000$\backslash$25  & 0.749 & 0.521  & 0.780 & 0.780 & 0.790 & \textbf{0.793}  \\ %  
\hline
% Credit Default & UCIrvine & C  &  30000$\backslash$25 & 0.782 &  0.678  & 0.799  & 0.792  &  0.813 & \textbf{0.822}   \\  % 
Credit Default & UCIrvine & C  &  30000$\backslash$25 & 0.782 &  0.678  & 0.815 & 0.812  &  0.819 & \textbf{0.822}   \\  % 
\hline
% Messidor features & UCIrvine & C & 1150$\backslash$19  & 0.743 &  0.731  & 0.762 & 0.756 & 0.781 & \textbf{0.793}     \\  % 
Messidor features & UCIrvine & C & 1150$\backslash$19  & 0.743 &  0.731  & 0.757 & 0.756 & 0.781 & \textbf{0.793}     \\  % 
\hline
% Wine Quality Red & UCIrvine & C & 999$\backslash$12  & 0.671  &  0.387 & 0.708 & 0.691  &  0.716  & \textbf{0.723}   \\  % 
Wine Quality Red & UCIrvine & C & 999$\backslash$12  & 0.671  &  0.387 & 0.692 & 0.691  &  0.716  & \textbf{0.723}   \\  % 
\hline
% Wine Quality White & UCIrvine & C &  4900$\backslash$12  & 0.652 &  0.371 & 0.707 & 0.701  &  0.708  & \textbf{0.708}  \\ % 
Wine Quality White & UCIrvine & C &  4900$\backslash$12  & 0.652 &  0.371 & 0.687 & 0.671  &  0.708  & \textbf{0.708}  \\ % 
\hline
% SpamBase & UCIrvine  & C & 4601$\backslash$57  & 0.940 &  0.939 &  0.948 &  0.945 &  0.949 & \textbf{0.949}  \\  % 
SpamBase & UCIrvine  & C & 4601$\backslash$57  & 0.934 &  0.939 &  0.938 &  0.935 &  0.949 & \textbf{0.949}  \\  % 
\hline
% table 2
% AP-omentum-lung & OpenML  & C & 203$\backslash$10936  & 0.962 & 0.944 & 0.981 & 0.974 & 0.983 & \textbf{0.985}  \\  % 
AP-omentum-lung & OpenML  & C & 203$\backslash$10936  & 0.962 & 0.944 & 0.966 & 0.964 & 0.983 & \textbf{0.985}  \\  % 
\hline
% credit-a & UCIrvine & C &  690$\backslash$6 & 0.782 &  0.798 & 0.803 & 0.789 &  0.810 & \textbf{0.815} \\  % 
credit-a & UCIrvine & C &  690$\backslash$6 & 0.782 &  0.798 & 0.793 & 0.789 &  0.810 & \textbf{0.815} \\  % 
\hline
% diabetes & UCIrvine & C &   768$\backslash$8  & 0.778 & 0.695  & 0.786  & 0.784 & 0.798 & \textbf{0.798}   \\  %   
diabetes & UCIrvine & C &   768$\backslash$8  & 0.778 & 0.695  & 0.784  & 0.782 & 0.798 & \textbf{0.798}   \\  %   
\hline
% fertility & UCIrvine & C &   100$\backslash$9  & 0.896 &  0.474  & 0.913 & 0.912  &  0.916 & \textbf{0.920}   \\ % 
fertility & UCIrvine & C &   100$\backslash$9  & 0.896 &  0.474  & 0.900 & 0.900  &  0.916 & \textbf{0.920}   \\ %
\hline
% gisette & UCIrvine & C &  2100$\backslash$5000  & 0.953 &  0.950  & 0.959  & 0.959  &  0.971  & \textbf{0.978}    \\ % 
gisette & UCIrvine & C &  2100$\backslash$5000  & 0.951 &  0.950  & 0.952  & 0.950  &  0.971  & \textbf{0.978}    \\ % 
\hline
% hepatitis & UCIrvine  & C &  155$\backslash$6  & 0.877 & 0.162 & 0.905 &  0.893 &  0.910 & \textbf{0.910}   \\  % 
hepatitis & UCIrvine  & C &  155$\backslash$6  & 0.877 & 0.162 & 0.884 &  0.873 &  0.910 & \textbf{0.910}   \\  % 
\hline
% labor & UCIrvine & C &  57$\backslash$8  & 0.876 &   0.862  & 0.960  &  0.950 & 0.964 & \textbf{0.964}  \\  % 
labor & UCIrvine & C &  57$\backslash$8  & 0.876 &   0.862  & 0.930  &  0.930 & 0.964 & \textbf{0.964}  \\  % 
\hline
% lymph & OpenML  & C & 138$\backslash$10936 & 0.971 &  1.000  & 0.987 & 0.978  & 0.992 & \textbf{1.000}    \\  % 
lymph & OpenML  & C & 138$\backslash$10936 & 0.961 &  1.000  & 0.964 & 0.964  & 0.992 & \textbf{1.000}    \\  % 
\hline
% madelon & UCIrvine & C &  780$\backslash$500  & 0.812 & 0.564  & 0.836 & 0.825  &  0.860 & \textbf{0.872}   \\  % 
madelon & UCIrvine & C &  780$\backslash$500  & 0.742 & 0.564  & 0.751 & 0.740  &  0.860 & \textbf{0.867}   \\  %  
\hline
% megawatt1 & UCIrvine & C &  253$\backslash$37  & 0.899 & 0.620 & 0.933  &  0.926 &  0.943  & \textbf{0.945}  \\ %  
megawatt1 & UCIrvine & C &  253$\backslash$37  & 0.899 & 0.620 & 0.913  &  0.904 &  0.943  & \textbf{0.945}  \\ %  
\hline
% secom & UCIrvine & C &  470$\backslash$590  & 0.922 &  0.030  & \textbf{0.934} & 0.927 &  0.930  & 0.932   \\ %   
secom & UCIrvine & C &  470$\backslash$590  & 0.922 &  0.030  & 0.929 & 0.927 &  0.930  & \textbf{0.932}   \\ % 
\hline
% sonar & UCIrvine & C &  208$\backslash$60  & 0.810 &  0.699   & 0.839 & 0.834  & 0.849 & \textbf{0.851}   \\ %
sonar & UCIrvine & C &  208$\backslash$60  & 0.740 &  0.699   & 0.770 & 0.768  & 0.840 & \textbf{0.842}   \\ %
\hline
\end{tabular}
\caption{Comparison results on 36 target datasets. C$\backslash$R is the downstream type. C is classification. R is regression. $\mathrm{RTDL_{RN}}$ is ResNet with RF from RTDL \cite{gorishniy2021revisiting}. $\mathrm{AutoFS_{RD}}$ \cite{fan2020autofs,fan2020interactive} is feature selection from randomly generated features. $\mathrm{NFS}$ \cite{chen2019neural} is feature generation and evaluation. $\TheName _{RD}$ is the ablation study of ~\TheName~, replacing the approximate hashing model with a random dropout method. $\TheName _{RL}$ is the ablation study of ~\TheName~, replacing the RL framework with policy gradient method like $\mathrm{NFS}$ \cite{chen2019neural} used.}
\label{tab:comparsion_score}
\end{table*}

==> features.table.tex <==
\begin{table}
\centering
\caption{Comparison of feature evaluation numbers of one epoch in the target dataset. $\mathrm{AutoFS_{R}}$ ($\mathrm{FS_{R}}$) \cite{fan2020autofs,fan2020interactive} is feature selection from randomly generated features. $\mathrm{NFS}$ \cite{chen2019neural} is feature generation and evaluation. $\TheName _{D}$ is the ablation study of ~\TheName~, replacing the approximate hashing model with a random dropout method.}
\begin{adjustbox}{scale=0.65}
\begin{tabular}{c|l|l|l|l|c|l|l|l|l}
\hline
Dataset & $\mathrm{FS_{R}}$  & NFS  & $\TheName _{D}$ & \TheName & Dataset & $\mathrm{FS_{R}}$ & NFS  & $\TheName _{D}$  & \TheName \\
\hline
Higgs Boson & 4640 & 4585 & 2273  & \textbf{2182} &  Openml 586 & 4000 & 3891 & 1996 & \textbf{932} \\  %  
\hline
A. Employee & 1440 & 1322 & 667 & \textbf{603} & Credit Default & 3680 & 3593 & 1823 & \textbf{1608} \\  % 
\hline
PimaIndian & 1280  & 1230 & 585 & \textbf{474} &  Messidor features & 3040 & 2958 & 1470 & \textbf{1448}   \\  % 
\hline
SpectF & 7040 & 6964 & 3372 & \textbf{3116} &  Wine Q. Red & 1760 & 1665 & 867 &  \textbf{806} \\  % 
\hline
SVMGuide3 & 3360 & 3269 & 1577 & \textbf{1573} &  Wine Q. White & 1760  & 1646 & 849 & \textbf{596}  \\  % 
\hline
German Credit & 3840 & 3748 & 1634 & \textbf{1473} &  SpamBase & 9120 & 9016 & 4347 & \textbf{4015}  \\  % 
\hline
Bikeshare DC & 1600  & 1537 & 743  & \textbf{327} & AP. lung & 8000 & 7905 & \textbf{3954} & 3966 \\  % 
\hline
Housing Boston & 1920 & 1826 & 898  & \textbf{559} & credit-a & 960 & 898 & \textbf{415} & 483  \\  % 
\hline
Airfoil & 800 & 698 & 333 & \textbf{161} & diabetes & 1280 & 1208 & 589 &  \textbf{489} \\  % 
\hline
AP. ovary & 8000 & 7905 & \textbf{3937} & 4008 &  fertility & 1440 & 1361 & 670 &  \textbf{552}  \\  % 
\hline
Lymphography & 2880 & 2809 & 1339 & \textbf{1160} & gisette & 8000 & 7875 & 3954 & \textbf{3667}  \\  % 
\hline
Ionosphere & 5440 & 5364 & 2600 & \textbf{2139} &  hepatitis & 960 & 836 & 407 & \textbf{363}  \\  % 
\hline
Openml 618 & 8000 & 7905 & 3903 & \textbf{1572} &  labor & 1280 & 1202 & \textbf{596} &  695  \\  % 
\hline
Openml 589 & 4000 & 3889 & 1934 & \textbf{975} &  lymph & 8000 & 7891 & 4042 &  \textbf{4033}  \\  % 
\hline
Openml 616 & 8000 & 7917 & 3967 & \textbf{2009} &  madelon & 8000 & 7923 & 3549 &  \textbf{3549} \\  % 
\hline
Openml 607 & 8000 & 7900 & 3960 & \textbf{1671} &  megawatt1 & 5760 & 5695 & 2845 &  \textbf{2319}  \\  % 
\hline
Openml 620 & 4000 & 3883 & 1924 & \textbf{929} &  secom & 3200 & 3087 & \textbf{1559} & 1647 \\  % 
\hline
Openml 637 & 8000 & 7894 & 4040 & \textbf{2038} &  sonar & 9600 & 9501 & \textbf{4747} & 4762 \\  % 
\hline
\end{tabular}
\end{adjustbox}
\label{tab:feature_evaluated}
\end{table}

==> features.table2.tex <==
\begin{table*}
\centering
\caption{Comparison of feature evaluation numbers of one epoch in the target dataset. $\mathrm{AutoFS_{R}}$ ($\mathrm{FS_{R}}$) \cite{fan2020autofs,fan2020interactive} is feature selection from randomly generated features. $\mathrm{NFS}$ \cite{chen2019neural} is feature generation and evaluation. $\TheName _{D}$ is the ablation study of ~\TheName~, replacing the approximate hashing model with a random dropout method.}
\label{tab:feature_evaluated}
\begin{tabular}{c|l|l|l|l|l|l|l|c|l|l|l|l|l|l|l} 
\hline
Dataset        & $\mathrm{FS_{R}}$ & NFS  & $\TheName _D$ &  &  &  &               & Dataset           & $\mathrm{FS_{R}}$ & NFS  & $\TheName _D$ & $\TheName ^P$  & $\TheName ^I$ & $\TheName ^L$ &                \\ 
\hline
Higgs Boson    & 4640              & 4585 & 2273          &  &  &  & \textbf{2182} & Openml 586        & 4000              & 3891 & 1996          &  &  &  & \textbf{932}   \\ 
\hline
A. Employee    & 1440              & 1322 & 667           &  &  &  & \textbf{603}  & Credit Default    & 3680              & 3593 & 1823          &  &  &  & \textbf{1608}  \\ 
\hline
PimaIndian     & 1280              & 1230 & 585           &  &  &  & \textbf{474}  & Messidor features & 3040              & 2958 & 1470          &  &  &  & \textbf{1448}  \\ 
\hline
SpectF         & 7040              & 6964 & 3372          &  &  &  & \textbf{3116} & Wine Q. Red       & 1760              & 1665 & 867           &  &  &  & \textbf{806}   \\ 
\hline
SVMGuide3      & 3360              & 3269 & 1577          &  &  &  & \textbf{1573} & Wine Q. White     & 1760              & 1646 & 849           &  &  &  & \textbf{596}   \\ 
\hline
German Credit  & 3840              & 3748 & 1634          &  &  &  & \textbf{1473} & SpamBase          & 9120              & 9016 & 4347          &  &  &  & \textbf{4015}  \\ 
\hline
Bikeshare DC   & 1600              & 1537 & 743           &  &  &  & \textbf{327}  & AP. lung          & 8000              & 7905 & \textbf{3954} &  &  &  & 3966           \\ 
\hline
Housing Boston & 1920              & 1826 & 898           &  &  &  & \textbf{559}  & credit-a          & 960               & 898  & \textbf{415}  &  &  &  & 483            \\ 
\hline
Airfoil        & 800               & 698  & 333           &  &  &  & \textbf{161}  & diabetes          & 1280              & 1208 & 589           &  &  &  & \textbf{489}   \\ 
\hline
AP. ovary      & 8000              & 7905 & \textbf{3937} &  &  &  & 4008          & fertility         & 1440              & 1361 & 670           &  &  &  & \textbf{552}   \\ 
\hline
Lymphography   & 2880              & 2809 & 1339          &  &  &  & \textbf{1160} & gisette           & 8000              & 7875 & 3954          &  &  &  & \textbf{3667}  \\ 
\hline
Ionosphere     & 5440              & 5364 & 2600          &  &  &  & \textbf{2139} & hepatitis         & 960               & 836  & 407           &  &  &  & \textbf{363}   \\ 
\hline
Openml 618     & 8000              & 7905 & 3903          &  &  &  & \textbf{1572} & labor             & 1280              & 1202 & \textbf{596}  &  &  &  & 695            \\ 
\hline
Openml 589     & 4000              & 3889 & 1934          &  &  &  & \textbf{975}  & lymph             & 8000              & 7891 & 4042          &  &  &  & \textbf{4033}  \\ 
\hline
Openml 616     & 8000              & 7917 & 3967          &  &  &  & \textbf{2009} & madelon           & 8000              & 7923 & 3549          &  &  &  & \textbf{3549}  \\ 
\hline
Openml 607     & 8000              & 7900 & 3960          &  &  &  & \textbf{1671} & megawatt1         & 5760              & 5695 & 2845          &  &  &  & \textbf{2319}  \\ 
\hline
Openml 620     & 4000              & 3883 & 1924          &  &  &  & \textbf{929}  & secom             & 3200              & 3087 & \textbf{1559} &  &  &  & 1647           \\ 
\hline
Openml 637     & 8000              & 7894 & 4040          &  &  &  & \textbf{2038} & sonar             & 9600              & 9501 & \textbf{4747} &  &  &  & 4762           \\
\hline
\end{tabular}
\end{table*}

==> minhash.table3.tex <==
\begin{table*}
\centering
\caption{Comparison results on 36 target datasets. C$\backslash$R is the downstream type. C is classification. R is regression. $\mathrm{RTDL_{N}}$ ($\mathrm{DL_{N}}$) is ResNet with RF from RTDL \cite{gorishniy2021revisiting}. $\mathrm{AutoFS_{R}}$ ($\mathrm{FS_{R}}$) \cite{fan2020autofs,fan2020interactive} is feature selection from randomly generated features. $\mathrm{NFS}$ \cite{chen2019neural} is feature generation and evaluation. $\TheName _{D}$ is the ablation study of ~\TheName~, replacing the approximate hashing model with a random dropout method. $\TheName _{R}$ is the ablation study of ~\TheName~, replacing the RL framework with policy gradient method like $\mathrm{NFS}$ \cite{chen2019neural} used. $\TheName ^{P}$ is $\TheName$ with PCWS \cite{wu2017consistent}. $\TheName ^{I}$ is $\TheName$ with ICWS \cite{ioffe2010improved}. $\TheName ^{L}$ is $\TheName$ with LICWS \cite{li20150-bit}.
$\TheName$ use CCWS \cite{wu2016canonical}}
\label{tab:comparsion_score}
% \begin{adjustbox}{scale=1.0}
\begin{tabular}{c|c|l|l|l|l|l|l|l|c|l|l|l} 
\hline
Dataset            & Source   & \begin{tabular}[c]{@{}l@{}}C$\backslash$\\R\end{tabular} & \begin{tabular}[c]{@{}l@{}}Samples$\backslash$\\Features\end{tabular} & $\mathrm{FS_{R}}$ & $\mathrm{DL_{N}}$ & NFS   & $\TheName _{R}$ & $\TheName _{D}$ &  $\TheName ^{L}$   &  $\TheName ^{P}$   & $\TheName ^{I}$               &     \TheName           \\ 
\hline
Higgs Boson       & UCIrvine & C                                                        & 50000$\backslash$28                                                   & 0.723             & 0.756             & 0.731 & 0.725         & 0.802         & 0.821 & 0.833 & 0.816 & \textbf{0.836}  \\ 
\hline
A. Employee       & Kaggle   & C                                                        & 32769$\backslash$9                                                    & 0.948             & 0.484             & 0.950 & 0.943         & 0.950         & 0.950 & 0.951 & 0.950 & \textbf{0.951}  \\ 
\hline
PimaIndian        & UCIrvine & C                                                        & 768$\backslash$8                                                      & 0.779             & 0.743             & 0.790 & 0.783         & 0.792         & 0.793 & 0.797 & 0.795 & \textbf{0.798}  \\ 
\hline
SpectF            & UCIrvine & C                                                        & 267$\backslash$44                                                     & 0.871             & 0.639             & 0.876 & 0.862         & 0.900         & 0.903 & 0.900 & 0.892 & \textbf{0.903}  \\ 
\hline
SVMGuide3         & LibSVM   & C                                                        & 1243$\backslash$21                                                    & 0.842             & 0.728             & 0.846 & 0.843         & 0.875         & 0.872 & 0.879 & 0.881 & \textbf{0.881}  \\ 
\hline
German Credit     & UCIrvine & C                                                        & 1001$\backslash$24                                                    & 0.775             & 0.681             & 0.780 & 0.773         & 0.810         & 0.796 & 0.816 & 0.813 & \textbf{0.816}  \\ 
\hline
Bikeshare DC      & Kaggle   & R                                                        & 10886$\backslash$11                                                   & 0.978             & 0.945             & 0.990 & 0.983         & 0.992         & 0.991 & 0.993 & 0.993 & \textbf{0.993}  \\ 
\hline
Housing Boston    & UCIrvine & R                                                        & 506$\backslash$13                                                     & 0.709             & 0.648             & 0.710 & 0.693         & 0.798         & 0.813 & 0.819 & 0.817 & \textbf{0.821}  \\ 
\hline
Airfoil           & UCIrvine & R                                                        & 1503$\backslash$5                                                     & 0.784             & 0.697             & 0.796 & 0.781         & 0.790         & 0.795 & 0.810 & 0.807 & \textbf{0.810}  \\ 
\hline
AP. ovary         & OpenML   & C                                                        & 275$\backslash$10936                                                  & 0.852             & 0.659             & 0.864 & 0.858         & 0.879         & 0.880 & 0.876 & 0.879 & \textbf{0.884}  \\ 
\hline
Lymphography      & UCIrvine & C                                                        & 148$\backslash$18                                                     & 0.895             & 0.000             & 0.922 & 0.921         & 0.960         & 0.958 & 0.960 & 0.961 & \textbf{0.964}  \\ 
\hline
Ionosphere        & UCIrvine & C                                                        & 351$\backslash$34                                                     & 0.934             & 0.883             & 0.957 & 0.944         & 0.973         & 0.977 & 0.964 & 0.970 & \textbf{0.977}  \\ 
\hline
Openml 618        & OpenML   & R                                                        & 1000$\backslash$50                                                    & 0.619             & 0.072             & 0.640 & 0.635         & 0.728         & 0.729 & 0.731 & 0.737 & \textbf{0.737}  \\ 
\hline
Openml 589        & OpenML   & R                                                        & 1000$\backslash$25                                                    & 0.737             & 0.578             & 0.754 & 0.748         & 0.757         & 0.754 & 0.762 & 0.762 & \textbf{0.764}  \\ 
\hline
Openml 616        & OpenML   & R                                                        & 500$\backslash$50                                                     & 0.609             & 0.000             & 0.673 & 0.653         & 0.675         & 0.676 & 0.689 & 0.680 & \textbf{0.689}  \\ 
\hline
Openml 607        & OpenML   & R                                                        & 1000$\backslash$50                                                    & 0.634             & 0.025             & 0.688 & 0.678         & 0.728         & 0.729 & 0.727 & 0.733 & \textbf{0.734}  \\ 
\hline
Openml 620        & OpenML   & R                                                        & 1000$\backslash$25                                                    & 0.705             & 0.047             & 0.732 & 0.727         & 0.736         & 0.734 & 0.747 & 0.741 & \textbf{0.748}  \\ 
\hline
Openml 637        & OpenML   & R                                                        & 500$\backslash$50                                                     & 0.608             & 0.016             & 0.634 & 0.633         & 0.624         & 0.635 & 0.642 & 0.636 & \textbf{0.646}  \\ 
\hline
Openml 586        & OpenML   & R                                                        & 1000$\backslash$25                                                    & 0.749             & 0.521             & 0.780 & 0.780         & 0.790         & 0.793 & 0.781 & 0.784 & \textbf{0.793}  \\ 
\hline
Credit Default    & UCIrvine & C                                                        & 30000$\backslash$25                                                   & 0.782             & 0.678             & 0.815 & 0.812         & 0.819         & 0.821 & 0.821 & 0.816 & \textbf{0.822}  \\ 
\hline
Messidor features & UCIrvine & C                                                        & 1150$\backslash$19                                                    & 0.743             & 0.731             & 0.757 & 0.756         & 0.781         & 0.783 & 0.790 & 0.784 & \textbf{0.793}  \\ 
\hline
Wine Q. Red       & UCIrvine & C                                                        & 999$\backslash$12                                                     & 0.671             & 0.387             & 0.692 & 0.691         & 0.716         & 0.717 & 0.720 & 0.723 & \textbf{0.723}  \\ 
\hline
Wine Q. White     & UCIrvine & C                                                        & 4900$\backslash$12                                                    & 0.652             & 0.371             & 0.687 & 0.671         & 0.708         & 0.708 & 0.705 & 0.708 & \textbf{0.708}  \\ 
\hline
SpamBase          & UCIrvine & C                                                        & 4601$\backslash$57                                                    & 0.934             & 0.939             & 0.938 & 0.935         & 0.949         & 0.949 & 0.949 & 0.944 & \textbf{0.949}  \\ 
\hline
AP. lung          & OpenML   & C                                                        & 203$\backslash$10936                                                  & 0.962             & 0.944             & 0.966 & 0.964         & 0.983         & 0.985 & 0.979 & 0.985 & \textbf{0.985}  \\ 
\hline
credit-a          & UCIrvine & C                                                        & 690$\backslash$6                                                      & 0.782             & 0.798             & 0.793 & 0.789         & 0.810         & 0.814 & 0.893 & 0.815 & \textbf{0.815}  \\ 
\hline
diabetes          & UCIrvine & C                                                        & 768$\backslash$8                                                      & 0.778             & 0.695             & 0.784 & 0.782         & 0.798         & 0.798 & 0.781 & 0.784 & \textbf{0.798}  \\ 
\hline
fertility         & UCIrvine & C                                                        & 100$\backslash$9                                                      & 0.896             & 0.474             & 0.900 & 0.900         & 0.916         & 0.911 & 0.919 & 0.913 & \textbf{0.920}  \\ 
\hline
gisette           & UCIrvine & C                                                        & 2100$\backslash$5000                                                  & 0.951             & 0.950             & 0.952 & 0.950         & 0.971         & 0.973 & 0.969 & 0.978 & \textbf{0.978}  \\ 
\hline
hepatitis         & UCIrvine & C                                                        & 155$\backslash$6                                                      & 0.877             & 0.162             & 0.884 & 0.873         & 0.910         & 0.894 & 0.910 & 0.887 & \textbf{0.910}  \\ 
\hline
labor             & UCIrvine & C                                                        & 57$\backslash$8                                                       & 0.876             & 0.862             & 0.930 & 0.930         & 0.964         & 0.957 & 0.960 & 0.960 & \textbf{0.964}  \\ 
\hline
lymph             & OpenML   & C                                                        & 138$\backslash$10936                                                  & 0.961             & 1.000             & 0.964 & 0.964         & 0.992         & 1.000 & 0.990 & 0.994 & \textbf{1.000}  \\ 
\hline
madelon           & UCIrvine & C                                                        & 780$\backslash$500                                                    & 0.742             & 0.564             & 0.751 & 0.740         & 0.860         & 0.860 & 0.864 & 0.864 & \textbf{0.867}  \\ 
\hline
megawatt1         & UCIrvine & C                                                        & 253$\backslash$37                                                     & 0.899             & 0.620             & 0.913 & 0.904         & 0.943         & 0.941 & 0.937 & 0.942 & \textbf{0.945}  \\ 
\hline
secom             & UCIrvine & C                                                        & 470$\backslash$590                                                    & 0.922             & 0.030             & 0.929 & 0.927         & 0.930         & 0.929 & 0.932 & 0.932 & \textbf{0.932}  \\ 
\hline
sonar             & UCIrvine & C                                                        & 208$\backslash$60                                                     & 0.740             & 0.699             & 0.770 & 0.768         & 0.840         & 0.842 & 0.833 & 0.837 & \textbf{0.842}  \\
\hline
\end{tabular}
% \end{adjustbox}
\end{table*}

==> variants.table.tex <==
\begin{table*}
\centering
\caption{Comparison of feature evaluation numbers of one epoch in the target dataset. $\mathrm{AutoFS_{R}}$ ($\mathrm{FS_{R}}$) \cite{fan2020autofs,fan2020interactive} is feature selection from randomly generated features. $\mathrm{NFS}$ \cite{chen2019neural} is feature generation and evaluation. $\TheName _{D}$ is the ablation study of ~\TheName~, replacing the approximate hashing model with a random dropout method.}
\begin{tabular}{c|l|l|l|l|c|l|l|l|l}
\hline
Dataset & $\mathrm{FS_{R}}$  & NFS  & $\TheName _{D}$ & \TheName & Dataset & $\mathrm{FS_{R}}$ & NFS  & $\TheName _{D}$  & \TheName \\
\hline
Higgs Boson & 4640 & 4585 & 2273  & \textbf{2182} &  Openml 586 & 4000 & 3891 & 1996 & \textbf{932} \\  %  
\hline
A. Employee & 1440 & 1322 & 667 & \textbf{603} & Credit Default & 3680 & 3593 & 1823 & \textbf{1608} \\  % 
\hline
PimaIndian & 1280  & 1230 & 585 & \textbf{474} &  Messidor features & 3040 & 2958 & 1470 & \textbf{1448}   \\  % 
\hline
SpectF & 7040 & 6964 & 3372 & \textbf{3116} &  Wine Q. Red & 1760 & 1665 & 867 &  \textbf{806} \\  % 
\hline
SVMGuide3 & 3360 & 3269 & 1577 & \textbf{1573} &  Wine Q. White & 1760  & 1646 & 849 & \textbf{596}  \\  % 
\hline
German Credit & 3840 & 3748 & 1634 & \textbf{1473} &  SpamBase & 9120 & 9016 & 4347 & \textbf{4015}  \\  % 
\hline
Bikeshare DC & 1600  & 1537 & 743  & \textbf{327} & AP. lung & 8000 & 7905 & \textbf{3954} & 3966 \\  % 
\hline
Housing Boston & 1920 & 1826 & 898  & \textbf{559} & credit-a & 960 & 898 & \textbf{415} & 483  \\  % 
\hline
Airfoil & 800 & 698 & 333 & \textbf{161} & diabetes & 1280 & 1208 & 589 &  \textbf{489} \\  % 
\hline
AP. ovary & 8000 & 7905 & \textbf{3937} & 4008 &  fertility & 1440 & 1361 & 670 &  \textbf{552}  \\  % 
\hline
Lymphography & 2880 & 2809 & 1339 & \textbf{1160} & gisette & 8000 & 7875 & 3954 & \textbf{3667}  \\  % 
\hline
Ionosphere & 5440 & 5364 & 2600 & \textbf{2139} &  hepatitis & 960 & 836 & 407 & \textbf{363}  \\  % 
\hline
Openml 618 & 8000 & 7905 & 3903 & \textbf{1572} &  labor & 1280 & 1202 & \textbf{596} &  695  \\  % 
\hline
Openml 589 & 4000 & 3889 & 1934 & \textbf{975} &  lymph & 8000 & 7891 & 4042 &  \textbf{4033}  \\  % 
\hline
Openml 616 & 8000 & 7917 & 3967 & \textbf{2009} &  madelon & 8000 & 7923 & 3549 &  \textbf{3549} \\  % 
\hline
Openml 607 & 8000 & 7900 & 3960 & \textbf{1671} &  megawatt1 & 5760 & 5695 & 2845 &  \textbf{2319}  \\  % 
\hline
Openml 620 & 4000 & 3883 & 1924 & \textbf{929} &  secom & 3200 & 3087 & \textbf{1559} & 1647 \\  % 
\hline
Openml 637 & 8000 & 7894 & 4040 & \textbf{2038} &  sonar & 9600 & 9501 & \textbf{4747} & 4762 \\  % 
\hline
\end{tabular}
\label{tab:variants}
\end{table*}
